Human-Aligned Skill Discovery: Balancing Behaviour Exploration and Alignment

Unsupervised skill discovery in Reinforcement Learning aims to mimic humans' ability to autonomously discover diverse behaviors. However, existing methods are often unconstrained, making it difficult to find useful skills, especially in complex environments, where discovered skills are frequently unsafe or impractical. We address this issue by proposing Human-aligned Skill Discovery (HaSD), a framework that incorporates human feedback to discover safer, more aligned skills. HaSD simultaneously optimises skill diversity and alignment with human values. This approach ensures that alignment is maintained throughout the skill discovery process, eliminating the inefficiencies associated with exploring unaligned skills. We demonstrate its effectiveness in both 2D navigation and SafetyGymnasium environments, showing that HaSD discovers diverse, human-aligned skills that are safe and useful for downstream tasks. Finally, we extend HaSD by learning a range of configurable skills with varying degrees of diversity alignment trade-offs that could be useful in practical scenarios.

==> paper/experiments/sections/safety_gymnasium/introduction.tex <==
\begin{figure}[htbp]
    \begin{subfigure}[b]{0.085\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper/experiments/figures/safety_gymnasium/figures/point_front.pdf} 
        \caption{Point}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.085\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper/experiments/figures/safety_gymnasium/figures/car_front.pdf} 
        \caption{Car}
    \end{subfigure}
    \hfill
        \begin{subfigure}[b]{0.085\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper/experiments/figures/safety_gymnasium/figures/racecar_front.pdf} 
        \caption{Racecar}
    \end{subfigure} 
    \hfill 
    \begin{subfigure}[b]{0.085\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper/experiments/figures/safety_gymnasium/figures/doggo_front.pdf} 
        \caption{Doggo}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.085\textwidth}
        \centering
        \includegraphics[width=\textwidth]{paper/experiments/figures/safety_gymnasium/figures/ant_front.pdf} 
        \caption{Ant}
    \end{subfigure}
    \hfill
    \caption{Range of agents used to evaluate our method on safety gymnasium.}
    \label{fig: safety_gymnasium agents}
    \Description{Range of agents used to evaluate our method on safety gymnasium.}
\end{figure}
\begin{figure}[htbp]
    \begin{subfigure}[b]{0.20\textwidth}
        \centering
       \includegraphics[width=\linewidth]{paper/experiments/figures/safety_gymnasium/figures/avoid_task.pdf} 
        \caption{Hazardous-Room}
        \label{fig: Hazardous-Room environment}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.20\textwidth}
        \centering
        \includegraphics[width=\linewidth]{paper/experiments/figures/safety_gymnasium/figures/push_task.pdf} 
        \caption{Push-Room}
        \label{fig: Push-Room environment}
    \end{subfigure}
    \caption{(a) In the Hazardous-Room environment, the agent should ideally avoid the purple circles while navigating. (b) In the Push-Room environment, the agent should ideally move the yellow box around the room.}
    \label{fig: safety_gymnasium  environment}
    \Description{(a) In the Hazardous-Room environment, the agent should ideally avoid the purple circles while navigating. (b) In the Push-Room environment, the agent should ideally move the yellow box around the room.}
\end{figure}


